Bayesian Optimal Data Detector for Hybrid mmWave MIMO-OFDM Systems with Low-Resolution ADCs

Hybrid analog-digital precoding architectures and low-resolution analog-to-digital converter (ADC) receivers are two solutions to reduce hardware cost and power consumption for millimeter wave (mmWave) multiple-input multiple-output (MIMO) communication systems with large antenna arrays. In this study, we consider a mmWave MIMO-OFDM receiver with a generalized hybrid architecture in which a small number of radio-frequency (RF) chains and low-resolution ADCs are employed simultaneously. Owing to the strong nonlinearity introduced by low-resolution ADCs, the task of data detection is challenging, particularly achieving a Bayesian optimal data detector. This study aims to fill this gap. By using generalized expectation consistent signal recovery technique, we propose a computationally efficient data detection algorithm that provides a minimum mean-square error estimate on data symbols and is extended to a mixed-ADC architecture. Considering particular structure of MIMO-OFDM channel matirx, we provide a lowcomplexity realization in which only FFT operation and matrixvector multiplications are required. Furthermore, we present an analytical framework to study the theoretical performance of the detector in the large-system limit, which can precisely evaluate the performance expressions such as mean-square error and symbol error rate. Based on this optimal detector, the potential of adding a few low-resolution RF chains and high-resolution ADCs for mixed-ADC architecture is investigated. Simulation results confirm the accuracy of our theoretical analysis and can be used for system design rapidly. The results reveal that adding a few low-resolution RF chains to original unquantized systems can obtain significant gains.

==> macro.tex <==

%ÖÐÎĘËüc·û̖
\def\oo{\nolinebreak[4]\hspace{.3em}\raise.7ex\hbox{¡£}\hspace{0.3em}}
\def\pp{\nolinebreak[4]\hspace{.3em}\raise.8ex\hbox{£¬}\hspace{0.3em}}
\def\dd{\nolinebreak[4]\hspace{.3em}\raise.8ex\hbox{¡¢}\hspace{0.3em}}
\def\mm{\nolinebreak[4]\hspace{.3em}\raise.3ex\hbox{£»}\hspace{0.3em}}
\def\gg{\nolinebreak[4]\hspace{.3em}\raise.3ex\hbox{£º}\hspace{0.3em}}
\def\iu{\nolinebreak[4]\hspace{.3em}\raise.3ex\hbox{¡º}\hspace{0.3em}}
\def\id{\nolinebreak[4]\hspace{.3em}\raise.3ex\hbox{¡»}\hspace{0.3em}}

\renewcommand\thesection{\Roman{section}.}
\renewcommand\thesubsection{\Alph{subsection}.}
\renewcommand\thesubsubsection{\Alph{subsection}.\arabic{subsubsection}}
%arabic °¢À­²®"µ×Ö
%roman СŒ'µÄÁ_ñR"µ×Ö
%Roman ´óŒ'µÄÁ_ñR"µ×Ö
%alph СŒ'×Öĸ
%Alph ´óŒ'×Öĸ

%\renewcommand{\tablename}{\ctxfr ±í}
%\renewcommand{\figurename}{\ctxfr ˆD}
%\renewcommand{\contentsname}{\ctxfk Ä¿ä›}
%\renewcommand\refname{…¢¿¼ÎÄ«I}

    \newcommand{\qa}{{\bf a}}
    \newcommand{\qb}{{\bf b}}
    \newcommand{\qc}{{\bf c}}
    \newcommand{\qd}{{\bf d}}
    \newcommand{\qe}{{\bf e}}
    \newcommand{\qf}{{\bf f}}
    \newcommand{\qg}{{\bf g}}
    \newcommand{\qh}{{\bf h}}
    \newcommand{\qi}{{\bf i}}
    \newcommand{\qj}{{\bf j}}
    \newcommand{\qk}{{\bf k}}
    \newcommand{\ql}{{\bf l}}
    \newcommand{\qm}{{\bf m}}
    \newcommand{\qn}{{\bf n}}
    \newcommand{\qo}{{\bf o}}
    \newcommand{\qp}{{\bf p}}
    \newcommand{\qq}{{\bf q}}
    \newcommand{\qr}{{\bf r}}
    \newcommand{\qs}{{\bf s}}
    \newcommand{\qt}{{\bf t}}
    \newcommand{\qu}{{\bf u}}
    \newcommand{\qv}{{\bf v}}
    \newcommand{\qw}{{\bf w}}
    \newcommand{\qx}{{\bf x}}
    \newcommand{\qy}{{\bf y}}
    \newcommand{\qz}{{\bf z}}

    \newcommand{\qA}{{\bf A}}
    \newcommand{\qB}{{\bf B}}
    \newcommand{\qC}{{\bf C}}
    \newcommand{\qD}{{\bf D}}
    \newcommand{\qE}{{\bf E}}
    \newcommand{\qF}{{\bf F}}
    \newcommand{\qG}{{\bf G}}
    \newcommand{\qH}{{\bf H}}
    \newcommand{\qI}{{\bf I}}
    \newcommand{\qJ}{{\bf J}}
    \newcommand{\qK}{{\bf K}}
    \newcommand{\qL}{{\bf L}}
    \newcommand{\qM}{{\bf M}}
    \newcommand{\qN}{{\bf N}}
    \newcommand{\qO}{{\bf O}}
    \newcommand{\qP}{{\bf P}}
    \newcommand{\qQ}{{\bf Q}}
    \newcommand{\qR}{{\bf R}}
    \newcommand{\qS}{{\bf S}}
    \newcommand{\qT}{{\bf T}}
    \newcommand{\qU}{{\bf U}}
    \newcommand{\qV}{{\bf V}}
    \newcommand{\qW}{{\bf W}}
    \newcommand{\qX}{{\bf X}}
    \newcommand{\qY}{{\bf Y}}
    \newcommand{\qZ}{{\bf Z}}
    \newcommand{\qzero}{{\bf 0}}
    \newcommand{\qdh}{\triangle\qh}
    \newcommand{\qhh}{\hat\qh}
    \newcommand{\qdH}{\triangle\qH}
    \newcommand{\qhH}{\hat\qH}
    \newcommand{\qdF}{\triangle\qF}
    \newcommand{\qhF}{\hat\qF}
    \newcommand{\qbh}{\bar\qh}
    \newcommand{\qbn}{\bar\qn}

    %\newcommand{\tr}{\mbox{trace}}
    \def\bm#1{\boldsymbol{#1}}

    \def\Complex{{\rm\rule[.23ex]{.03em}{1.1ex}\kern-.3em{C}}}
    \def\bms#1{\mbox{\boldmath $\scriptstyle #1$}}


    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\beas}{\begin{eqnarray*}} \newcommand{\eeas}{\end{eqnarray*}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof : }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof : }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  %\newtheorem{theorem}{Theorem}
  %\newtheorem{conjecture}{Conjecture}
  %\newtheorem{definition}{Definition}
  %\newtheorem{example}{Example}
  %\newtheorem{lemma}{Lemma}
  %\newtheorem{proposition}{Proposition}
  %\newtheorem{claim}{Claim}

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

    %%%%%% DEFINITION %%%%%%%%%%%%%%
    \newcommand{\bbE}{{\mathbb E}}
    \newcommand{\bbR}{{\mathbb R}}
    \newcommand{\bbC}{{\mathbb C}}
    \newcommand{\bbS}{{\mathbb S}}
    \newcommand{\bbF}{{\mathbb F}}

    \newcommand{\calA}{{\mathcal A}}
    \newcommand{\calD}{{\mathcal D}}
    \newcommand{\calE}{{\mathcal E}}
    \newcommand{\calF}{{\mathcal F}}
    \newcommand{\calK}{{\mathcal K}}
    \newcommand{\calL}{{\mathcal L}}
    \newcommand{\calN}{{\mathcal N}}
    \newcommand{\calI}{{\mathcal I}}
    \newcommand{\calO}{{\mathcal O}}

    \newcommand{\dom}{{\tt dom}}
    \newcommand{\epi}{{\tt epi}}
    \newcommand{\diag}{{\tt diag}}
    \newcommand{\supp}{{\tt supp}}
    \newcommand{\tr}{{\sf tr}}
    \newcommand{\Ex}{{\sf E}}
    \newcommand{\rank}{{\sf rank}}

    \newcommand{\bfbl}[1]{\bf \color{blue}#1}
    \newcommand{\bfrl}[1]{\bf \color{red}#1}
    \newcommand{\bfbrl}[1]{\bf \color{BrickRed}#1}
    \newcommand{\bfbbl}[1]{\bf \color{BlueViolet}#1}


    \newcommand{\mnorm}[1]{|\!|\!|#1|\!|\!|}
    \newcommand{\innp}[1]{\langle #1 \rangle}

    \newcommand{\qDelta}{{\boldsymbol \Delta}}
    \newcommand{\qPsi}{{\boldsymbol \Psi}}
    \newcommand{\qPhi}{{\boldsymbol \Phi}}
    \newcommand{\qXi}{{\boldsymbol \Xi}}
    \newcommand{\qTheta}{{\boldsymbol \Theta}}
    \newcommand{\qLambda}{{\boldsymbol \Lambda}}

    \newcommand{\qalpha}{{\boldsymbol \alpha}}
    \newcommand{\qbeta}{{\boldsymbol \beta}}
    \newcommand{\qlambda}{{\boldsymbol \lambda}}
    \newcommand{\qgamma}{{\boldsymbol \gamma}}
    \newcommand{\qepsilon}{{\boldsymbol \epsilon}}

    \newcommand{\bbCnn}{{\mathbb C}^{n \times n}}
    \newcommand{\bbCn}{{\mathbb C}^{n}}
    \newcommand{\bbRnn}{{\mathbb R}^{n \times n}}
    \newcommand{\bbRn}{{\mathbb R}^{n}}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

